Mitigating Bias in Calibration Error Estimation

For an AI system to be reliable, the confidence it expresses in its decisions must match its accuracy. To assess the degree of match, examples are typically binned by confidence and the per-bin mean confidence and accuracy are compared. Most research in calibration focuses on techniques to reduce this empirical measure of calibration error, ECE_bin. We instead focus on assessing statistical bias in this empirical measure, and we identify better estimators. We propose a framework through which we can compute the bias of a particular estimator for an evaluation data set of a given size. The framework involves synthesizing model outputs that have the same statistics as common neural architectures on popular data sets. We find that binning-based estimators with bins of equal mass (number of instances) have lower bias than estimators with bins of equal width. Our results indicate two reliable calibration-error estimators: the debiased estimator (Brocker, 2012; Ferro and Fricker, 2012) and a method we propose, ECE_sweep, which uses equal-mass bins and chooses the number of bins to be as large as possible while preserving monotonicity in the calibration function. With these estimators, we observe improvements in the effectiveness of recalibration methods and in the detection of model miscalibration.

==> Mitigating bias in calibration error estimation/latexdefs.tex <==
  
\newcommand{\dist}{\ensuremath{\mathcal{D}}}
\newcommand{\fhat}{\ensuremath{\hat{f}}}
\newcommand{\ermloss}{\ensuremath{L}}
\newcommand{\Eop}{\ensuremath{\mathop{\mathbb{E}}}}
\newcommand{\E}{\Eop}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\N}{\ensuremath{\mathcal{N}}}
\newcommand{\prob}{\ensuremath{\mathbb{P}}}
\newcommand{\Dtest}{\ensuremath{S}}
\newcommand{\D}[1]{\ensuremath{D_{\text{#1}}}}
\newcommand{\ind}{\ensuremath{\mathbb{I}}}
\newcommand{\acc}{\ensuremath{\text{acc}}}
\newcommand{\Beta}{\ensuremath{\text{Beta}}}
\newcommand{\Uniform}{\ensuremath{\text{Uniform}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\model}[1]{\texttt{#1}}
\newcommand{\metric}[1]{\texttt{#1}}
% \newcommand{\ewmonsweep}{\metric{ew\_mon\_sweep}}
% \newcommand{\emmonsweep}{\metric{em\_mon\_sweep}}
% \newcommand{\ewece}{\metric{ew\_ece}}
% \newcommand{\emece}{\metric{em\_ece}}

\newcommand{\ewmonsweep}{\ensuremath{\text{ECE}^\textsc{ew}_\textsc{sweep}}}
\newcommand{\emmonsweep}{\ensuremath{\text{ECE}^\textsc{em}_\textsc{sweep}}}
\newcommand{\emdebias}{\ensuremath{\text{ECE}^\textsc{em}_\textsc{debias}}}
\newcommand{\ewdebias}{\ensuremath{\text{ECE}^\textsc{ew}_\textsc{debias}}}
\newcommand{\kde}{\ensuremath{\text{KDE}}}
\newcommand{\ewece}{\ensuremath{\text{ECE}^\textsc{ew}_\textsc{bin}}}
\newcommand{\emece}{\ensuremath{\text{ECE}^\textsc{em}_\textsc{bin}}}
\newcommand{\EM}{{\textsc{em}}}
\newcommand{\EW}{{\textsc{ew}}}

%\newcommand{\ewmonsweep}{\color{red}\texttt{EWsweep}}
%\newcommand{\emmonsweep}{\color{red}\texttt{EMsweep}}
%\newcommand{\emdebias}{\color{red}\texttt{EMdebias}}
%\newcommand{\kde}{\color{red}\texttt{KDE}}
%\newcommand{\ewece}{\color{red}\texttt{EW}}
%\newcommand{\emece}{\color{red}\texttt{EM}}

\newcommand{\ecebin}{\ensuremath{{\text{ECE}_{\textsc{bin}}}}}
\newcommand{\ecedebias}{\ensuremath{{\text{ECE}_{\textsc{debias}}}}}
\newcommand{\celb}{\ensuremath{{\text{ECE}_{\textsc{lb}}}}}
\newcommand{\cesweep}{\ensuremath{{\text{ECE}_{\textsc{sweep}}}}}
\newcommand{\BBC}{{BBC}}

\newcommand{\ceneighborhood}{\ensuremath{{\text{ECE}_{\mathcal{N}}}}}

\newcommand{\avgce}{\ensuremath{{\langle{\text{ECE}}\rangle}}}
\newcommand{\truecurve}{\ensuremath{\E_Y[Y \mid f(X)=c]}}
\newcommand{\truecurvex}{\ensuremath{\E_Y[Y \mid f(X)]}}
\newcommand{\truece}{\ensuremath{\text{true calibration error}}}
\newcommand{\tce}{\ensuremath{\text{TCE}}}


\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

%\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
%\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
%\DeclarePairedDelimiter{\parens}{\lparen}{\rparen}
%\DeclarePairedDelimiter{\brackets}{[}{]}
%\DeclarePairedDelimiter{\ip}{\langle}{\rangle}

\iftoggle{showtodos}{
\newcommand{\becca}[1]{\todo[color=green!40]{Becca: #1}}
\newcommand{\nick}[1]{\todo[color=blue!40]{Nick: #1}}
\newcommand{\mike}[1]{\todo[color=red!40]{Mike: #1}}
\newcommand{\jon}[1]{\todo[color=purple!40]{Jon: #1}}
}{
\newcommand{\becca}[1]{}
\newcommand{\nick}[1]{}
\newcommand{\jon}[1]{}
\newcommand{\mike}[1]{}
}
\newcommand{\testtext}[1]{\color{magenta!95}#1 }


==> Mitigating bias in calibration error estimation/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> Mitigating bias in calibration error estimation/tables/beta_dist_data.tex <==
\begin{table}[ht!]
\centering
\caption{Parameters of best fit for Beta distribution investigated in Section \ref{sec:glm_beta_fits}.}
\label{table:beta_fit_data}
\begin{tabular}{lrr}
\toprule
{} &  $\hat{\alpha}$ &  $\hat{\beta}$ \\
\midrule
resnet110\_c10      &     2.7752 &    0.0478 \\
resnet110\_SD\_c10   &     2.1714 &    0.0394 \\
resnet\_wide32\_c10  &     2.3806 &    0.0379 \\
densenet40\_c10     &     1.9824 &    0.0397 \\
resnet110\_c100     &     1.1823 &    0.1081 \\
resnet110\_SD\_c100  &     1.1233 &    0.1147 \\
resnet\_wide32\_c100 &     1.0611 &    0.0650 \\
densenet40\_c100    &     1.0805 &    0.0808 \\
resnet152\_imgnet   &     1.1359 &    0.2069 \\
densenet161\_imgnet &     1.1928 &    0.2206 \\
\bottomrule
\end{tabular}
\end{table}


==> Mitigating bias in calibration error estimation/tables/eece_sece_data.tex <==
\begin{table}[ht!]
\centering
\caption{\ecebin{} reported in Figure \ref{fig:beta_glm_fit}c.}
\label{table:eece_sece}
\begin{tabular}{lrr}
\toprule
{} &  \ecebin{} (\%) &  <\ecebin{}> (\%, simulated) \\
\midrule
resnet110\_c10      &     6.67 &     8.42 \\
resnet110\_SD\_c10   &     6.54 &     8.79 \\
resnet\_wide32\_c10  &     6.09 &     8.44 \\
densenet40\_c10     &     6.70 &     8.09 \\
resnet110\_c100     &    20.26 &    18.87 \\
resnet110\_SD\_c100  &    17.44 &    15.78 \\
resnet\_wide32\_c100 &    20.40 &    17.53 \\
densenet40\_c100    &    23.12 &    19.69 \\
resnet152\_imgnet   &     6.85 &     9.26 \\
densenet161\_imgnet &     6.15 &     6.87 \\
\bottomrule
\end{tabular}
\end{table}


==> Mitigating bias in calibration error estimation/tables/glm_fit_data_0.tex <==
\begin{tabular}{llrrr}
\toprule
               &            &                         AIC &  $b_{0}$ &  $b_{1}$ \\
dataset\_name & glm\_name &                             &         &         \\
\midrule
resnet110\_c10 & logflip\_logflip\_b0\_b1 & \textbf{2779.22} &   -0.24 &    0.30 \\
               & logit\_logflip\_b0\_b1 &                     2790.40 &   -0.55 &   -0.38 \\
               & logit\_logflip\_b1 &                     2827.51 &      &   -0.31 \\
               & logit\_logit\_b0\_b1 &                     2840.70 &   -0.38 &    0.36 \\
               & logit\_logit\_b1 &                     2900.02 &      &    0.30 \\
               & logflip\_logflip\_b1 &                     2932.09 &      &    0.34 \\
               & log\_log\_b0\_b1 &                     3221.72 &   -0.06 &    2.53 \\
               & logit\_logit\_b0 &                     3799.63 &    1.99 &      \\
               & logflip\_logflip\_b0 &                     3811.98 &   -2.13 &      \\
               & log\_log\_b0 &                     3829.05 &   -0.13 &      \\
               & logit\_logflip\_b0 &                     3868.40 &    1.95 &      \\
               & log\_log\_b1 &                     4281.78 &      &    4.75 \\
resnet110\_SD\_c10 & logit\_logflip\_b0\_b1 & \textbf{2498.98} &   -0.27 &   -0.35 \\
               & logit\_logit\_b1 &                     2502.52 &      &    0.30 \\
               & logit\_logflip\_b1 &                     2508.70 &      &   -0.30 \\
               & logit\_logit\_b0\_b1 &                     2538.41 &   -0.26 &    0.33 \\
               & logflip\_logflip\_b0\_b1 &                     2550.29 &   -0.36 &    0.27 \\
               & logflip\_logflip\_b1 &                     2572.85 &      &    0.35 \\
               & log\_log\_b0\_b1 &                     2594.91 &   -0.08 &    1.98 \\
               & log\_log\_b0 &                     3137.19 &   -0.19 &      \\
               & logflip\_logflip\_b0 &                     3150.42 &   -1.80 &      \\
               & logit\_logit\_b0 &                     3175.58 &    1.58 &      \\
               & logit\_logflip\_b0 &                     3179.67 &    1.56 &      \\
               & log\_log\_b1 &                     3697.37 &      &    3.77 \\
resnet\_wide32\_c10 & logit\_logit\_b1 & \textbf{2483.34} &      &    0.26 \\
               & logflip\_logflip\_b0\_b1 &                     2487.69 &   -0.47 &    0.22 \\
               & logit\_logit\_b0\_b1 &                     2511.39 &   -0.13 &    0.28 \\
               & logit\_logflip\_b0\_b1 &                     2558.45 &   -0.26 &   -0.28 \\
               & logit\_logflip\_b1 &                     2586.47 &      &   -0.25 \\
               & log\_log\_b0\_b1 &                     2647.03 &   -0.12 &    1.87 \\
               & logflip\_logflip\_b1 &                     2713.17 &      &    0.30 \\
               & log\_log\_b0 &                     2981.24 &   -0.21 &      \\
               & logflip\_logflip\_b0 &                     2983.05 &   -1.70 &      \\
               & logit\_logit\_b0 &                     2989.90 &    1.49 &      \\
               & logit\_logflip\_b0 &                     3055.55 &    1.45 &      \\
               & log\_log\_b1 &                     4582.09 &      &    4.61 \\
densenet40\_c10 & logit\_logflip\_b1 & \textbf{2910.62} &      &   -0.26 \\
               & logit\_logit\_b0\_b1 &                     2961.31 &   -0.40 &    0.31 \\
               & logit\_logflip\_b0\_b1 &                     3000.23 &   -0.38 &   -0.31 \\
               & logflip\_logflip\_b0\_b1 &                     3001.78 &   -0.31 &    0.24 \\
               & logit\_logit\_b1 &                     3021.54 &      &    0.25 \\
               & logflip\_logflip\_b1 &                     3027.78 &      &    0.31 \\
               & log\_log\_b0\_b1 &                     3153.38 &   -0.12 &    2.04 \\
               & log\_log\_b0 &                     3531.22 &   -0.22 &      \\
               & logflip\_logflip\_b0 &                     3589.11 &   -1.60 &      \\
               & logit\_logit\_b0 &                     3601.85 &    1.37 &      \\
               & logit\_logflip\_b0 &                     3679.95 &    1.30 &      \\
               & log\_log\_b1 &                     4735.18 &      &    4.27 \\
resnet110\_c100 & logflip\_logflip\_b0\_b1 & \textbf{8181.97} &   -0.11 &    0.28 \\
               & logit\_logit\_b0\_b1 &                     8206.19 &   -0.88 &    0.39 \\
               & logflip\_logflip\_b1 &                     8301.28 &      &    0.31 \\
               & logit\_logflip\_b0\_b1 &                     8371.53 &   -1.01 &   -0.40 \\
               & logit\_logit\_b1 &                     8732.11 &      &    0.25 \\
               & log\_log\_b0\_b1 &                     8918.21 &   -0.16 &    2.35 \\
               & logit\_logflip\_b1 &                     8926.99 &      &   -0.23 \\
               & logit\_logflip\_b0 &                    10903.83 &    0.74 &      \\
               & logit\_logit\_b0 &                    10943.95 &    0.72 &      \\
               & logflip\_logflip\_b0 &                    10964.91 &   -1.12 &      \\
               & log\_log\_b0 &                    11002.20 &   -0.40 &      \\
               & log\_log\_b1 &                    11850.89 &      &    4.26 \\
\bottomrule
\end{tabular}


==> Mitigating bias in calibration error estimation/tables/glm_fit_data_1.tex <==
\begin{tabular}{llrrr}
\toprule
                   &            &                          AIC &  $b_{0}$ &  $b_{1}$ \\
dataset\_name & glm\_name &                              &         &         \\
\midrule
resnet110\_SD\_c100 & logit\_logit\_b0\_b1 &  \textbf{7873.61} &   -0.88 &    0.49 \\
                   & logflip\_logflip\_b0\_b1 &                      7878.19 &   -0.09 &    0.35 \\
                   & logflip\_logflip\_b1 &                      7932.28 &      &    0.38 \\
                   & logit\_logflip\_b0\_b1 &                      7944.61 &   -1.04 &   -0.52 \\
                   & logit\_logit\_b1 &                      8315.51 &      &    0.32 \\
                   & log\_log\_b0\_b1 &                      8437.82 &   -0.11 &    2.18 \\
                   & logit\_logflip\_b1 &                      8510.36 &      &   -0.30 \\
                   & log\_log\_b1 &                      9988.07 &      &    3.30 \\
                   & logit\_logit\_b0 &                     10803.27 &    0.80 &      \\
                   & log\_log\_b0 &                     10810.90 &   -0.37 &      \\
                   & logflip\_logflip\_b0 &                     10823.15 &   -1.16 &      \\
                   & logit\_logflip\_b0 &                     10834.48 &    0.78 &      \\
resnet\_wide32\_c100 & logflip\_logflip\_b0\_b1 &  \textbf{7183.93} &   -0.13 &    0.21 \\
                   & logit\_logit\_b0\_b1 &                      7219.14 &   -0.98 &    0.33 \\
                   & logflip\_logflip\_b1 &                      7233.51 &      &    0.25 \\
                   & logit\_logflip\_b0\_b1 &                      7297.00 &   -1.06 &   -0.34 \\
                   & logit\_logit\_b1 &                      7626.21 &      &    0.19 \\
                   & log\_log\_b0\_b1 &                      7650.97 &   -0.24 &    2.51 \\
                   & logit\_logflip\_b1 &                      7795.28 &      &   -0.17 \\
                   & logflip\_logflip\_b0 &                      8977.39 &   -0.98 &      \\
                   & logit\_logflip\_b0 &                      8987.38 &    0.49 &      \\
                   & log\_log\_b0 &                      9000.24 &   -0.49 &      \\
                   & logit\_logit\_b0 &                      9009.51 &    0.49 &      \\
                   & log\_log\_b1 &                     11911.51 &      &    5.48 \\
densenet40\_c100 & logit\_logit\_b0\_b1 &  \textbf{8158.28} &   -0.97 &    0.34 \\
                   & logflip\_logflip\_b0\_b1 &                      8229.43 &   -0.12 &    0.22 \\
                   & logit\_logflip\_b0\_b1 &                      8267.77 &   -1.08 &   -0.35 \\
                   & logflip\_logflip\_b1 &                      8368.86 &      &    0.25 \\
                   & logit\_logit\_b1 &                      8783.50 &      &    0.19 \\
                   & log\_log\_b0\_b1 &                      8832.20 &   -0.25 &    2.26 \\
                   & logit\_logflip\_b1 &                      8918.57 &      &   -0.18 \\
                   & logit\_logit\_b0 &                     10138.24 &    0.47 &      \\
                   & logit\_logflip\_b0 &                     10182.61 &    0.45 &      \\
                   & logflip\_logflip\_b0 &                     10242.15 &   -0.94 &      \\
                   & log\_log\_b0 &                     10261.01 &   -0.50 &      \\
                   & log\_log\_b1 &                     13322.10 &      &    5.25 \\
resnet152\_imgnet & logflip\_logflip\_b0\_b1 & \textbf{18729.85} &   -0.12 &    0.58 \\
                   & logit\_logit\_b0\_b1 &                     18783.22 &   -0.29 &    0.65 \\
                   & log\_log\_b0\_b1 &                     18785.44 &   -0.03 &    1.32 \\
                   & logflip\_logflip\_b1 &                     18872.14 &      &    0.65 \\
                   & logit\_logit\_b1 &                     19074.37 &      &    0.57 \\
                   & logit\_logflip\_b0\_b1 &                     19095.40 &   -0.82 &   -0.79 \\
                   & log\_log\_b1 &                     19840.25 &      &    1.53 \\
                   & logit\_logflip\_b1 &                     20062.10 &      &   -0.50 \\
                   & logflip\_logflip\_b0 &                     26935.09 &   -1.41 &      \\
                   & log\_log\_b0 &                     26968.50 &   -0.28 &      \\
                   & logit\_logflip\_b0 &                     27012.77 &    1.12 &      \\
                   & logit\_logit\_b0 &                     27084.11 &    1.11 &      \\
densenet161\_imgnet & log\_log\_b0\_b1 & \textbf{18202.41} &   -0.03 &    1.27 \\
                   & logit\_logit\_b0\_b1 &                     18460.70 &   -0.25 &    0.68 \\
                   & logflip\_logflip\_b1 &                     18521.48 &      &    0.67 \\
                   & logflip\_logflip\_b0\_b1 &                     18534.07 &   -0.10 &    0.61 \\
                   & logit\_logit\_b1 &                     18822.25 &      &    0.60 \\
                   & logit\_logflip\_b0\_b1 &                     18913.25 &   -0.77 &   -0.80 \\
                   & log\_log\_b1 &                     19493.85 &      &    1.44 \\
                   & logit\_logflip\_b1 &                     19562.58 &      &   -0.54 \\
                   & logit\_logflip\_b0 &                     26426.38 &    1.19 &      \\
                   & logflip\_logflip\_b0 &                     26445.91 &   -1.46 &      \\
                   & logit\_logit\_b0 &                     26519.76 &    1.18 &      \\
                   & log\_log\_b0 &                     26662.65 &   -0.27 &      \\
\bottomrule
\end{tabular}


==> Mitigating bias in calibration error estimation/tmp.tex <==
\begin{table}
\centering
\caption{Comparison of ECE values from \cite{guo2017calibration} versus ew\_ece\_bin (N=15 bins)}
\label{table:guo_vs_ew_ece_bin}
\begin{tabular}{lllrr}
\toprule
Uncalibrated ECE(\%) & x=Gou et al. & y=ew\_bin &    x-y & 100(x-y)/x \\
\midrule
     densenet40\_c10 &         3.28 &     5.50 &  -2.22 &     -67.69 \\
   resnet110\_SD\_c10 &         4.12 &     4.11 &   0.01 &       0.18 \\
  resnet\_wide32\_c10 &         4.52 &     4.51 &   0.01 &       0.32 \\
      resnet110\_c10 &         4.60 &     4.75 &  -0.15 &      -3.27 \\
   resnet152\_imgnet &         5.48 &     6.54 &  -1.06 &     -19.40 \\
 densenet161\_imgnet &         6.28 &     5.72 &   0.56 &       8.92 \\
    densenet40\_c100 &        10.37 &    21.16 & -10.79 &    -104.01 \\
  resnet110\_SD\_c100 &        12.67 &    15.86 &  -3.19 &     -25.18 \\
 resnet\_wide32\_c100 &        15.00 &    18.78 &  -3.78 &     -25.23 \\
     resnet110\_c100 &        16.53 &    18.48 &  -1.95 &     -11.80 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{Comparison of ECE values (and associated rank orderings) computed using ew\_ece\_bin vs em\_ece\_sweep from uncalibrated logits.}
\label{table:ew_ece_bin_em_ece_sweep}
\begin{tabular}{lllrr}
\toprule
Uncalibrated ECE(\%) &   x=ew\_bin & y=em\_sweep &   x-y & 100(x-y)/x \\
\midrule
   resnet110\_SD\_c10 &    4.11(0) &    4.10(0) &  0.01 &       0.24 \\
  resnet\_wide32\_c10 &    4.51(1) &    4.48(1) &  0.03 &       0.66 \\
      resnet110\_c10 &    4.75(2) &    4.75(2) & -0.00 &      -0.00 \\
     densenet40\_c10 &    5.50(3) &    5.49(3) &  0.01 &       0.13 \\
 densenet161\_imgnet &    5.72(4) &    5.72(4) & -0.00 &      -0.00 \\
   resnet152\_imgnet &    6.54(5) &    6.54(5) &  0.00 &       0.00 \\
  resnet110\_SD\_c100 &   15.86(6) &   15.83(6) &  0.03 &       0.18 \\
     resnet110\_c100 &   18.48(7) &   18.48(7) &  0.00 &       0.00 \\
 resnet\_wide32\_c100 &   18.78(8) &   18.78(8) & -0.00 &      -0.00 \\
    densenet40\_c100 &   21.16(9) &   21.16(9) &  0.00 &       0.00 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{Comparison of ECE values (and associated rank orderings) computed using ew\_ece\_bin vs em\_ece\_sweep from logits calibrated using temperature scaling \cite{guo2017calibration}. Red indicates differences in the sorted order of each entry in the column.}
\label{table:ew_ece_bin_ts_em_ece_sweep_ts}
\begin{tabular}{lllrr}
\toprule
   Temp. scaling(\%) &   x=ew\_bin &                   y=em\_sweep &   x-y & 100(x-y)/x \\
\midrule
   resnet110\_SD\_c10 &    0.56(0) &    0.36({\color{red}1}) &  0.19 &      34.99 \\
  resnet\_wide32\_c10 &    0.78(1) &    0.21({\color{red}0}) &  0.57 &      72.65 \\
    densenet40\_c100 &    0.90(2) &                      0.72(2) &  0.18 &      20.45 \\
     densenet40\_c10 &    0.95(3) &                      0.90(3) &  0.05 &       4.98 \\
      resnet110\_c10 &    1.13(4) &                      0.91(4) &  0.23 &      19.90 \\
  resnet110\_SD\_c100 &    1.21(5) &                      0.98(5) &  0.23 &      18.96 \\
 resnet\_wide32\_c100 &    1.47(6) &                      1.31(6) &  0.16 &      10.82 \\
 densenet161\_imgnet &    1.94(7) &    1.88({\color{red}8}) &  0.06 &       3.01 \\
   resnet152\_imgnet &    2.08(8) &    2.13({\color{red}9}) & -0.05 &      -2.59 \\
     resnet110\_c100 &    2.38(9) &    1.87({\color{red}7}) &  0.51 &      21.38 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{Comparison of ECE values (and associated rank orderings) computed using ew\_ece\_bin vs em\_ece\_sweep from logits calibrated using isotonic regression \cite{zadrozny2002transforming}.}
\label{table:ew_ece_bin_ir_em_ece_sweep_ir}
\begin{tabular}{lllrr}
\toprule
Isotonic regression(\%) &   x=ew\_bin & y=em\_sweep &   x-y & 100(x-y)/x \\
\midrule
      resnet110\_SD\_c10 &    1.03(0) &    0.70(0) &  0.33 &      32.15 \\
     resnet\_wide32\_c10 &    1.19(1) &    0.77(1) &  0.42 &      35.41 \\
         resnet110\_c10 &    1.47(2) &    0.93(2) &  0.55 &      37.14 \\
        densenet40\_c10 &    1.68(3) &    1.61(3) &  0.08 &       4.66 \\
    densenet161\_imgnet &    4.64(4) &    4.64(4) & -0.00 &      -0.00 \\
     resnet110\_SD\_c100 &    4.89(5) &    4.86(5) &  0.04 &       0.81 \\
       densenet40\_c100 &    5.01(6) &    4.95(6) &  0.06 &       1.14 \\
      resnet152\_imgnet &    5.15(7) &    5.11(7) &  0.04 &       0.74 \\
    resnet\_wide32\_c100 &    5.76(8) &    5.64(8) &  0.12 &       2.15 \\
        resnet110\_c100 &    6.19(9) &    6.05(9) &  0.15 &       2.40 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{Comparison of ECE values (and associated rank orderings) computed using ew\_ece\_bin vs em\_ece\_sweep from logits calibrated using histogram binning \cite{zadrozny2001obtaining}. Red indicates differences in the sorted order of each entry in the column.}
\label{table:ew_ece_bin_hb_em_ece_sweep_hb}
\begin{tabular}{lllrr}
\toprule
Histogram binning(\%) &   x=ew\_bin &                   y=em\_sweep &   x-y & 100(x-y)/x \\
\midrule
   resnet\_wide32\_c10 &    0.56(0) &                      0.56(0) &  0.00 &       0.00 \\
    resnet110\_SD\_c10 &    0.62(1) &                      0.57(1) &  0.05 &       7.61 \\
    resnet152\_imgnet &    0.78(2) &    0.76({\color{red}4}) &  0.02 &       2.14 \\
  densenet161\_imgnet &    0.80(3) &    0.64({\color{red}2}) &  0.16 &      19.86 \\
     densenet40\_c100 &    0.81(4) &    0.80({\color{red}5}) &  0.01 &       1.02 \\
       resnet110\_c10 &    0.84(5) &    0.67({\color{red}3}) &  0.17 &      20.67 \\
      resnet110\_c100 &    0.91(6) &                      0.91(6) &  0.00 &       0.00 \\
      densenet40\_c10 &    1.27(7) &                      1.27(7) & -0.00 &      -0.00 \\
  resnet\_wide32\_c100 &    1.45(8) &                      1.45(8) &  0.00 &       0.00 \\
   resnet110\_SD\_c100 &    1.58(9) &                      1.55(9) &  0.03 &       1.82 \\
\bottomrule
\end{tabular}
\end{table}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> tmp.tex <==
\begin{table}
\centering
\caption{Comparison of ECE values from \cite{guo2017calibration} versus ew\_ece\_bin (N=15 bins)}
\label{table:guo_vs_ew_ece_bin}
\begin{tabular}{lllrr}
\toprule
Uncalibrated ECE(\%) & x=Gou et al. & y=ew\_bin &    x-y & 100(x-y)/x \\
\midrule
     densenet40\_c10 &         3.28 &     5.50 &  -2.22 &     -67.69 \\
   resnet110\_SD\_c10 &         4.12 &     4.11 &   0.01 &       0.18 \\
  resnet\_wide32\_c10 &         4.52 &     4.51 &   0.01 &       0.32 \\
      resnet110\_c10 &         4.60 &     4.75 &  -0.15 &      -3.27 \\
   resnet152\_imgnet &         5.48 &     6.54 &  -1.06 &     -19.40 \\
 densenet161\_imgnet &         6.28 &     5.72 &   0.56 &       8.92 \\
    densenet40\_c100 &        10.37 &    21.16 & -10.79 &    -104.01 \\
  resnet110\_SD\_c100 &        12.67 &    15.86 &  -3.19 &     -25.18 \\
 resnet\_wide32\_c100 &        15.00 &    18.78 &  -3.78 &     -25.23 \\
     resnet110\_c100 &        16.53 &    18.48 &  -1.95 &     -11.80 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{Comparison of ECE values (and associated rank orderings) computed using ew\_ece\_bin vs em\_ece\_sweep from uncalibrated logits.}
\label{table:ew_ece_bin_em_ece_sweep}
\begin{tabular}{lllrr}
\toprule
Uncalibrated ECE(\%) &   x=ew\_bin & y=em\_sweep &   x-y & 100(x-y)/x \\
\midrule
   resnet110\_SD\_c10 &    4.11(0) &    4.10(0) &  0.01 &       0.24 \\
  resnet\_wide32\_c10 &    4.51(1) &    4.48(1) &  0.03 &       0.66 \\
      resnet110\_c10 &    4.75(2) &    4.75(2) & -0.00 &      -0.00 \\
     densenet40\_c10 &    5.50(3) &    5.49(3) &  0.01 &       0.13 \\
 densenet161\_imgnet &    5.72(4) &    5.72(4) & -0.00 &      -0.00 \\
   resnet152\_imgnet &    6.54(5) &    6.54(5) &  0.00 &       0.00 \\
  resnet110\_SD\_c100 &   15.86(6) &   15.83(6) &  0.03 &       0.18 \\
     resnet110\_c100 &   18.48(7) &   18.48(7) &  0.00 &       0.00 \\
 resnet\_wide32\_c100 &   18.78(8) &   18.78(8) & -0.00 &      -0.00 \\
    densenet40\_c100 &   21.16(9) &   21.16(9) &  0.00 &       0.00 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{Comparison of ECE values (and associated rank orderings) computed using ew\_ece\_bin vs em\_ece\_sweep from logits calibrated using temperature scaling \cite{guo2017calibration}. Red indicates differences in the sorted order of each entry in the column.}
\label{table:ew_ece_bin_ts_em_ece_sweep_ts}
\begin{tabular}{lllrr}
\toprule
   Temp. scaling(\%) &   x=ew\_bin &                   y=em\_sweep &   x-y & 100(x-y)/x \\
\midrule
   resnet110\_SD\_c10 &    0.56(0) &    0.36({\color{red}1}) &  0.19 &      34.99 \\
  resnet\_wide32\_c10 &    0.78(1) &    0.21({\color{red}0}) &  0.57 &      72.65 \\
    densenet40\_c100 &    0.90(2) &                      0.72(2) &  0.18 &      20.45 \\
     densenet40\_c10 &    0.95(3) &                      0.90(3) &  0.05 &       4.98 \\
      resnet110\_c10 &    1.13(4) &                      0.91(4) &  0.23 &      19.90 \\
  resnet110\_SD\_c100 &    1.21(5) &                      0.98(5) &  0.23 &      18.96 \\
 resnet\_wide32\_c100 &    1.47(6) &                      1.31(6) &  0.16 &      10.82 \\
 densenet161\_imgnet &    1.94(7) &    1.88({\color{red}8}) &  0.06 &       3.01 \\
   resnet152\_imgnet &    2.08(8) &    2.13({\color{red}9}) & -0.05 &      -2.59 \\
     resnet110\_c100 &    2.38(9) &    1.87({\color{red}7}) &  0.51 &      21.38 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{Comparison of ECE values (and associated rank orderings) computed using ew\_ece\_bin vs em\_ece\_sweep from logits calibrated using isotonic regression \cite{zadrozny2002transforming}.}
\label{table:ew_ece_bin_ir_em_ece_sweep_ir}
\begin{tabular}{lllrr}
\toprule
Isotonic regression(\%) &   x=ew\_bin & y=em\_sweep &   x-y & 100(x-y)/x \\
\midrule
      resnet110\_SD\_c10 &    1.03(0) &    0.70(0) &  0.33 &      32.15 \\
     resnet\_wide32\_c10 &    1.19(1) &    0.77(1) &  0.42 &      35.41 \\
         resnet110\_c10 &    1.47(2) &    0.93(2) &  0.55 &      37.14 \\
        densenet40\_c10 &    1.68(3) &    1.61(3) &  0.08 &       4.66 \\
    densenet161\_imgnet &    4.64(4) &    4.64(4) & -0.00 &      -0.00 \\
     resnet110\_SD\_c100 &    4.89(5) &    4.86(5) &  0.04 &       0.81 \\
       densenet40\_c100 &    5.01(6) &    4.95(6) &  0.06 &       1.14 \\
      resnet152\_imgnet &    5.15(7) &    5.11(7) &  0.04 &       0.74 \\
    resnet\_wide32\_c100 &    5.76(8) &    5.64(8) &  0.12 &       2.15 \\
        resnet110\_c100 &    6.19(9) &    6.05(9) &  0.15 &       2.40 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{Comparison of ECE values (and associated rank orderings) computed using ew\_ece\_bin vs em\_ece\_sweep from logits calibrated using histogram binning \cite{zadrozny2001obtaining}. Red indicates differences in the sorted order of each entry in the column.}
\label{table:ew_ece_bin_hb_em_ece_sweep_hb}
\begin{tabular}{lllrr}
\toprule
Histogram binning(\%) &   x=ew\_bin &                   y=em\_sweep &   x-y & 100(x-y)/x \\
\midrule
   resnet\_wide32\_c10 &    0.56(0) &                      0.56(0) &  0.00 &       0.00 \\
    resnet110\_SD\_c10 &    0.62(1) &                      0.57(1) &  0.05 &       7.61 \\
    resnet152\_imgnet &    0.78(2) &    0.76({\color{red}4}) &  0.02 &       2.14 \\
  densenet161\_imgnet &    0.80(3) &    0.64({\color{red}2}) &  0.16 &      19.86 \\
     densenet40\_c100 &    0.81(4) &    0.80({\color{red}5}) &  0.01 &       1.02 \\
       resnet110\_c10 &    0.84(5) &    0.67({\color{red}3}) &  0.17 &      20.67 \\
      resnet110\_c100 &    0.91(6) &                      0.91(6) &  0.00 &       0.00 \\
      densenet40\_c10 &    1.27(7) &                      1.27(7) & -0.00 &      -0.00 \\
  resnet\_wide32\_c100 &    1.45(8) &                      1.45(8) &  0.00 &       0.00 \\
   resnet110\_SD\_c100 &    1.58(9) &                      1.55(9) &  0.03 &       1.82 \\
\bottomrule
\end{tabular}
\end{table}

